Data Sharing Markets

With the growing use of distributed machine learning techniques, there is a growing need for data markets that allows agents to share data with each other. Nevertheless data has unique features that separates it from other commodities including replicability, cost of sharing, and ability to distort. We study a setup where each agent can be both buyer and seller of data. For this setup, we consider two cases: bilateral data exchange (trading data with data) and unilateral data exchange (trading data with money). We model bilateral sharing as a network formation game and show the existence of strongly stable outcome under the top agents property by allowing limited complementarity. We propose ordered match algorithm which can find the stable outcome in O(N^2) (N is the number of agents). For the unilateral sharing, under the assumption of additive cost structure, we construct competitive prices that can implement any social welfare maximizing outcome. Finally for this setup when agents have private information, we propose mixed-VCG mechanism which uses zero cost data distortion of data sharing with its isolated impact to achieve budget balance while truthfully implementing socially optimal outcomes to the exact level of budget imbalance of standard VCG mechanisms. Mixed-VCG uses data distortions as data money for this purpose. We further relax zero cost data distortion assumption by proposing distorted-mixed-VCG. We also extend our model and results to data sharing via incremental inquiries and differential privacy costs.

==> Pricing.tex <==

\begin{assumption}
 If sharing is unidirectional, then agent $n$ shares his data with agent $m$, without agent $n$ accessing $m$'s data. 
\end{assumption}

Unidirectional vs bidirectional sharing will change the notion of stability and the results we present in Sections \ref{ssec: core} and \ref{ssec: comp}.

With unidirectional sharing, the edges are directional and an edge exists from $n$ to $m$ if $n$ shares his data with $m$.
\end{definition} 
The set of outcomes denoted by $\mathcal{G}$ has $2^{N\times (N-1)/2}$ members for the bidirectional sharing, and $2^{N(N-1)}$ members with directional sharing.




\begin{remark}
Assumption \ref{ass: utility structure 2} is required for results of Section \ref{ssec: core}. However, the results in \ref{ssec: comp} and \ref{ssec: mech} still hold untapped.
\end{remark}


\section{Results}\label{sec: results}
We first look into the existence of a stable outcome for the data sharing problem (Section \ref{ssec: core}). Second we extend the model by allowing monetary transfers (numeraire in the quasi-linear utility functions), and look into existence of prices that realize social welfare (Section \ref{ssec: comp}). Third, we extend the model by assuming agents' types are private information (information asymmetry), and design mechanisms run by an intermediary to implement socially welfare maximizing outcome (Section \ref{ssec: mech}).

\subsection{Stable Outcomes}\label{ssec: core}



Agent $n$'s type denoted by $\theta_n$ determines agent $n$'s preferences over sharing outcomes.

\begin{remark} The outcome of the ordered match algorithm is not core stable for unidirectional sharing. To see this consider an example with three agents, $d_1=1$, $d_2=2$ and $d_3=3$. The costs of sharing are $c_1=1, c_2=1.1, c_3=2.1$. Also $u(d, \theta_n)= d$ for $n=1,2,3$. The outcome of the ordered match algorithm is an empty graph. However, it is not core stable with unidirectional sharing, since the three agents can deviate to $G=\{13, 23, 21, 32\}$. Here there is a directional sharing circle between 1, 2, and 3 which benefits all. Finding an algorithm for core stable outcome with unidirectional sharing is challenging due to this type of behavior.
\end{remark}

Denote by $S^I_n$ and $S^O_n$ the set of agents that $n$ has access to their data and agents that have access to $n$'s data correspondingly. For the bidirectional sharing, we consider $S_n=(S_n^I, S_n^O)$. In the case of unidirectional sharing, $S^I_n=S^O_n$ and we refer to both simply by $S_n$.

==> notes.tex <==
\section{Notes}


